ECO: Edge-Cloud Optimization of 5G applications

Centralized cloud computing with 100+ milliseconds network latencies cannot meet the tens of milliseconds to sub-millisecond response times required for emerging 5G applications like autonomous driving, smart manufacturing, tactile internet, and augmented or virtual reality. We describe a new, dynamic runtime that enables such applications to make effective use of a 5G network, computing at the edge of this network, and resources in the centralized cloud, at all times. Our runtime continuously monitors the interaction among the microservices, estimates the data produced and exchanged among the microservices, and uses a novel graph min-cut algorithm to dynamically map the microservices to the edge or the cloud to satisfy application-specific response times. Our runtime also handles temporary network partitions, and maintains data consistency across the distributed fabric by using microservice proxies to reduce WAN bandwidth by an order of magnitude, all in an {\it application-specific manner} by leveraging knowledge about the application's functions, latency-critical pipelines and intermediate data. We illustrate the use of our runtime by successfully mapping two complex, representative real-world video analytics applications to the AWS/Verizon Wavelength edge-cloud architecture, and improving application response times by 2x when compared with a static edge-cloud implementation.

==> background.tex <==
\section{Background}
{\bf 5G applications:} Demand for edge computing is rising due to an increasing number of new applications that 
interact with humans in real-time. For such applications, consideration of a few human-related benchmarks is useful. The time to blink an eye is about 150 ms \cite{eye-blink}, and a world-class sprinter can react within 120 ms of a starting gun \cite{sprinter}. The human auditory reaction time is about 100 ms, and the typical human visual reaction time is in the range of 10 ms \cite{human-reaction-time}. Also, nerve impulses travel at over 100 meters per second in the human body \cite{nerve-conduction}, and the time required to propagate a signal from hand to brain is about 10 ms \cite{brain-to-arm}. If application response times are in this range, then it is possible to interact with distant objects with no perceived difference to interactions with a local object. 
% Faster, 1-millisecond reaction time is required when a human is expecting speed, such as when remotely controlling a visual scene and issuing
% commands that anticipate rapid response.
%(like moving a mouse pointer over a screen, or moving the head while wearing Virtual Reality googles)
Even faster, sub-milliseconds response times are required for machine to machine communication as in industry 4.0, where closed-loop real-time control systems automate processes like quality control, high-speed manufacturing, food packaging, construction, and e-health, without the involvement of any human.  Clearly, if applications are to approach this level of responsiveness, the network latencies (not including processing) must be much less than 100 ms, which 5G network and edge computing can deliver.

\begin{figure}[t]
\centering
    \includegraphics[width=0.9\linewidth]{images/wavelength-infrastructure.png}
    \caption{AWS Wavelength Infrastructure}
    \lFig{wavelength-infrastructure}
\end{figure}

\begin{table}[b]
\caption{AWS Wavelength instance types}
\begin{center}
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
     \makecell{Instance \\ Types} & \makecell{vCPUs} & \makecell{Memory \\ (GiB)} & \makecell{GPU} &  \makecell{Network \\ Perf. \\ (Gigabit)} & \makecell{Price \\ (per hour)}\\
    \hline
    t3.medium & 2 & 4 & no & upto 5 & \$0.056\\
    \hline
    t3.xlarge & 4 & 16 & no &  upto 5 & \$0.224\\
    \hline
    r5.2xlarge & 8 & 64 & no &  upto 10 & \$0.68\\
    \hline
    g4dn.2xlarge & 8 & 32 & \makecell{yes} & upto 25 & \$1.317\\
    \hline
    \end{tabular}
\end{center}
\lTable{aws-wl-instances-types}
\end{table}

{\bf AWS Wavelength\cite{aws-wavelength}:}
%\section{AWS Wavelength Overview}
We use AWS Wavelength to explore edge-cloud solutions for 5G applications, in which
%Amazon has partnered with communication service providers like Verizon, Vodafone, KDDI and SK Telecom to offer this service in various parts of the world, including United States, Europe, Japan and Korea. 
AWS compute and storage is placed directly within the communication provider's network. 
%For example, AWS and Verizon have embedded AWS compute and storage services within Verizon's metro aggregation sites, which are at the edge of Verizon's 5G network. Unlike accessing the cloud using traditional mobile architectures, which requires several hops on the network (from a device, to a cell tower, to metro aggregation sites, to regional aggregation sites, to the Internet, to the cloud - and then back through those hops to get back to the device), application traffic only needs to travel from the device to a cell tower to a Wavelength Zone running in a metro aggregation site. 
This removes the latency that results from multiple hops between regional aggregation sites and across the Internet, and enables new, low-latency applications.
%AWS Wavelength is a new infrastructure recently introduced by Amazon towards an effort to provide compute and storage at the edge for ultra low-latency applications. 
%Amazon has also partnered with communication service providers like Verizon, Vodafone, KDDI and SK Telecom to offer this service in various parts of the world, including United States, Europe, Japan and Korea. To achieve ultra low-latency, AWS compute and storage is placed directly within the data centers of these telecom provider's network. This AWS infrastructure inside carrier network forms the Wavelength zone and applications can take full advantage of the latency and bandwidth offered by 5G, by having direct communication to 5G devices from within the same carrier network. 
%Amazon now has five available Wavelength Zones in United States:  Atlanta, Boston, New York City, Washington DC and San Francisco Bay area. 
%All these wavelength zones are in Verizon's network. AWS Wavelength currently supports four types of computing instances: t3.medium, t3.xlarge, r5.2xlarge and g4dn.2xlarge. \rTable{aws-wl-instances-types} shows the configuration for various instance types. Only g4dn.2xlarge instance has a GPU (Tesla T4). 
\rTable{aws-wl-instances-types} shows the configuration for various instance types available in AWS Wavelength.
A typical AWS Wavelength infrastructure is shown in \rFig{wavelength-infrastructure}, where the Amazon Virtual Private Cloud (VPC) is extended to include the Wavelength Zone and supported EC2 instances are spawned in the Wavelength zone to handle latency-sensitive  application components. 5G devices in the carrier network connect to the Wavelength Zone through the carrier gateway and network traffic from these devices is directly routed to the VMs in Wavelength zone without leaving the carrier network. 

%Once in Wavelength zone, data can be processed locally within Wavelength zone for latency-sensitive components and less-latency sensitive components or components that need to be shared across zones or components that need to persist state e.g. databases, can be run in the region.

%\begin{table}[b]
%\caption{AWS Wavelength instance types}
%\begin{center}
%    \begin{tabular}{|l|c|c|c|c|c|c|}
%    \hline
%     \makecell{Instance \\ Types} & \makecell{vCPUs} & \makecell{Memory \\ (GiB)} & \makecell{GPU} & \makecell{Storage} & \makecell{Network \\ Perf. \\ (Gigabit)} & \makecell{Price \\ (per hour)}\\
%    \hline
%    t3.medium & 2 & 4 & no & \makecell{EBS} & upto 5 & \$0.056\\
%    \hline
%    t3.xlarge & 4 & 16 & no & \makecell{EBS} & upto 5 & \$0.224\\
%    \hline
%    r5.2xlarge & 8 & 64 & no & \makecell{EBS} & upto 10 & \$0.68\\
%    \hline
%    g4dn.2xlarge & 8 & 32 & \makecell{yes} & \makecell{1x225 \\ (SSD)} & upto 25 & \$1.317\\
%    \hline
%    \end{tabular}
%\end{center}
%\lTable{aws-wl-instances-types}
%\end{table}

%Discuss overview of Verizon 5G, hotspots, their characteristics, limitations; AWS Wavelength overview, Wavelength VM characteristics, limitations;overall system architecture with Wavelength and 5G network.

==> centralized.tex <==
%\section{5G and AWS Wavelength test bed}
\section{Centralized delivery and management}
\rFig{centralized} shows a distributed architecture to handle deployments across different Wavelength zones, all from a centralized cloud. Users access a central site, and request for a set of services to be deployed on a collection of sensors. For example, in \rFig{centralized}, Alice from San Jose area contacts a VM in the Ohio Region zone, expressing an interest to start a particular application on a camera A (step 1). In response to the request, we create a VPC with appropriate Region and Wavelength zones for customers in San Jose area (steps 2 and 3). Then, the carrier gateway IP address, as well as the public IP address of the VM in the Oregon Region zone is sent back to Alice as a React progran, which points camera A to the carrier gateway IP address, and the service is now available on camera A.  Similarly, when Bob from New York wants to start a particular application on his camera B, he visits the central site in the Ohio Region zone and makes a request for a particular application on camera B (step 4). In response, we create another VPC with resources in the North Virginia Region zone and a Wavelength zone in New York (steps 5 and 6). Bob's camera B connects to the carrier gateway IP address for the Wavelength zone in New York, and avails the requested application. Our system can quickly set up such a global application service, without any human involvement.   
\subsubsection{Cloud Monitor (CM)}
Edge Monitor, described in \rSec{edge-monitor}, monitors application-level and network-level performance metrics at individual edge, while Cloud Monitor (CM) monitors and maintains this information from multiple edges, at a central location in the cloud. CM thus has a global view, while EM has a local view of the state of deployment of various applications. CM works in conjunction with EMs and maintains key edge-level metrics from individual edges and makes them available for Cloud Scheduler (CS) to make decisions about placement of applications at appropriate edges. Each EM, at periodic interval, reports edge-level metrics like health of the edge, performance of applications running on the edge, network performance between the edge and the cloud, etc., to CM, which then has the most up-to-date information from all the connected edges. If any of the edge looses connection due to network partitioning, then the information at CM from that edge is stale and subsequently CS avoids scheduling applications at that particular edge until network connection is restored. Alternatively, if the edge health seems to be unstable, then CM notes this and CS subsequently avoids scheduling applications on that edge until the edge health is back to normal.

\subsubsection{Cloud Scheduler (CS)}
Cloud Scheduler (CS) is the component that enables deployment of applications across different Wavelength zones. \rFig{cs-flow} shows the flowchart of the procedure followed by CS to serve a request for application deployment. Whenever a request to deploy a new application in a particular geographical region is received, CS first checks if there already exists an availability and wavelength zone setup for that region. If not, then a new VPC is created and availability and wavelength zone for the corresponding geographical region is setup. If a Wavelength zone is already setup, and is reachable (checked using data from CM), then it is selected for deployment of the application. After Wavelength zone, next is the selection or creation of VMs for application processing. If existing VMs can accomodate microservices of the application (checked using data from CM) then they are selected and if more VMs are needed for processing the application, then new VMs are created within the availability and wavelength zone. The health of these VMs is then checked using edge-level metrics from CM and if they look good, then application is deployed on these VMs and the request processing ends. If either the existing Wavelength zone is not reachable or the VMs are not in good health, an error is reported and request processing ends.

\begin{figure}[t]
\centering
    \includegraphics[width=0.6\linewidth]{images/cs-flow.png}
    \caption{Cloud Scheduler flowchart}
    \lFig{cs-flow}
\end{figure}

%Consider a web server deployed in Ohio region, which acts as the entry point for users from different geographical locations. Alice who resides in San Jose, sets up camera A in san Jose region (top right in \rFig{centralized}, connects to the centralized server and requests to start real-time monitoring application on camera A (step 1). Based on the identified location of Alice and the camera, from the centralized server, the closes region to Alice i.e. Oregon in this case is where the request processing is initiated (step 2), which then launches additional resources in "San Francisco Bay Area" Wavelength zone (step 3), which is closest to Alice, the entire pipeline is setup seamlessly and application processing starts right away and Alice is able to see the results from camera A. Simlarly, now Bob sets up camera B in New York (bottom right in \rFig{centralized}, and request to start monitoring camera B (step 4). Since Bob is in a different physical location, this time the region closest to him i.e. N. Virginia in this case is where the processing is initiated (step 5). This further launches resources in NYC wavelength zone (step 6), entire pipeline is setup and application processing for camera B starts seamlessly and results are available to Bob. With this kind of a deployment setup, the backend infrastructure is completely hidden to the end user and appropriate routing, and partitioning of tasks can be handled seamlessly.
 
%is when there is a centralized web server, as shown in \rFig{centralized} which receives the request for application processing, and depending on the physical location of the request, contacts the nearest region zone and wavelength zone to process the request. This way the backend infrastructure is completely hidden to the end user and appropriate routing, and partitioning of tasks can be handled seamlessly.

\begin{figure}[t]
   \includegraphics[width=0.999\linewidth]{images/centralized.png}
   \caption{Centralized application deployment (best option)}
   \lFig{centralized}
\end{figure}


==> large-scale-deployments.tex <==
\subsection{Large-scale deployments (cost estimate)}
\lSec{large-scale}
In this section, we provide cost estimates for deploying real-time monitoring application for a large-scale deployment i.e. 100-cameras deployment. \rTable{aws-cost-estimate} shows the AWS cost estimates using t3.xlarge instances in availability zone and wavelength zone. Cost for instances in availability zone and wavelength zone varies, for e.g. cost of t3.xlarge instance in availability zone, in this case US West (Oregon) is \$0.167 per hour while in wavelength zone, in this case US West (Verizon)-San Francisco Bay area, is \$0.224 per hour \cite{amazon-pricing-link}. 
%The higher cost at the wavelength zone comes with higher network bandwidth and lower latency to devices connected in the same carrier network. So, deployment with VMs in availability zone is cheaper but slower, while that on Wavelength zone is expensive but faster. 
On a t3.xlarge instance which has 4 vCPUs, we can run real-time monitoring application for 2 cameras. In this estimate, we did not include the data transfer cost because the price to get unlimited data IN to the EC2 instances in wavelength or availability zone is zero, and that to get upto 1 GB/month data OUT is also zero \cite{amazon-pricing-link}. The IN data is the video feeds and OUT data is the alerts, which are typically less than 1 GB/month. 

%For a deployment of 20 cameras with real-time monitoring application, we need 10 of the t3.xlarge VMs (since 1 VM can support 2 cameras). If we deploy purely on availability zone i.e. all application processing happens in availability zone, then the total cost (compute and storage) would be around \$1397.4 per month, while deploying it on Wavelength zone i.e. all application processing happens in the wavelength zone, will cost around \$2043.54, where we use 1 EC2 instance in Availability zone and 10 on Wavelength zone. In case of deployment in availability zone, the cameras connect directly to the VMs in availability zone, while in case of wavelength zone, cameras directly connect to the VMs in Wavelength zone through the carrier network. Along with these two, there is also a hybrid deployment, where cameras directly connect to VMs in the Wavelength zone through the carrier network, but the processing does not entirely happen there. Instead, the processing is split between VMs in availability zone and VMs in wavelength zone. The cost of such a hybrid deployment for a 20-camera setup is around \$1650.6 per month, which uses 5 EC2 instance in Wavelength zone and 5 instances in availability zone. 

The total cost for 100-camera deployment on availability zone is around \$6987 per month, while for deployment on wavelength zone is around \$9658.74. In both cases, 50 t3.xlarge instances are required for application processing, either in availability zone or wavelength zone. The cost for 100-camera hybrid deployment, with 25 instances in availability zone and 25 instances in wavelength zone is around \$8253. We note that the cost of hybrid deployment is lower than that of edge-only deployment i.e. on wavelength zone.

%Discuss various estimations for large-scale deployments (10 and 100 cameras);cost and latency for different architectures and design choices; what would the numbers be when all cameras are always active and what would it be when only some are active always and others are activated on-demand.
\begin{table*}[t]
\caption{Real-time monitoring application AWS cost estimate}
\begin{center}
    \begin{tabular}{|l|c|c|c|c|c|c|c|}
    \hline
     \makecell{Deployment \\ scenario} & \makecell{Number of \\cameras} & \makecell{Number of \\ Availability zone \\ instances (t3.xlarge)} & \makecell{Number of \\ Wavelength zone \\ instances (t3.xlarge)} & \makecell{Price \\ (per hour)} & \makecell{Compute price \\ (per month)} & \makecell{Storage price \\ (per month)} & \makecell{Total cost \\ (per month)}\\
    \hline
    %\makecell{Availability \\ Zone} & 1 & 1 & 0 & \$0.167 & \$120.24 & \$19.5 &  \$139.74\\
    %\makecell{Wavelength \\ Zone} & 1 & 1 & 1 & \$0.391 & \$281.52 & \$48.6 &  \$330.12\\
    %\makecell{Availability Zone} & 20 & 10 & 0 & \$1.67 & \$1202 & \$195 &  \$1397\\
    %\makecell{Wavelength Zone} & 20 & 1 & 10 & \$2.40 & \$1733.04 & \$310 &  \$2043\\
    %\makecell{Hybrid} & 20 & 5 & 5 & \$1.95 & \$1407 & \$243 & \$1650\\
    %\hline
    \makecell{Availability Zone} & 100 & 50 & 0 & \$8.35 & \$6012 & \$975 &  \$6987\\
    \makecell{Wavelength Zone} & 100 & 1 & 50 & \$11.37 & \$8184 & \$1474 &  \$9658 \\
    \makecell{Hybrid} & 100 & 25 & 25 & \$9.78 & \$7038 & \$1215 & \$8253\\
    \hline
    \end{tabular}
\end{center}
\lTable{aws-cost-estimate}
\end{table*}
